DDGHM: Dual Dynamic Graph with Hybrid Metric Training for Cross-Domain Sequential Recommendation

Sequential Recommendation (SR) characterizes evolving patterns of user behaviors by modeling how users transit among items. However, the short interaction sequences limit the performance of existing SR. To solve this problem, we focus on Cross-Domain Sequential Recommendation (CDSR) in this paper, which aims to leverage information from other domains to improve the sequential recommendation performance of a single domain. Solving CDSR is challenging. On the one hand, how to retain single domain preferences as well as integrate cross-domain influence remains an essential problem. On the other hand, the data sparsity problem cannot be totally solved by simply utilizing knowledge from other domains, due to the limited length of the merged sequences. To address the challenges, we propose DDGHM, a novel framework for the CDSR problem, which includes two main modules, i.e., dual dynamic graph modeling and hybrid metric training. The former captures intra-domain and inter-domain sequential transitions through dynamically constructing two-level graphs, i.e., the local graphs and the global graph, and incorporating them with a fuse attentive gating mechanism. The latter enhances user and item representations by employing hybrid metric learning, including collaborative metric for achieving alignment and contrastive metric for preserving uniformity, to further alleviate data sparsity issue and improve prediction accuracy. We conduct experiments on two benchmark datasets and the results demonstrate the effectiveness of DDHMG.

==> chapter/model-old.tex <==
\section{The Proposed Model}

In this section, we first formulate the cross-domain sequential recommendation (CDSR) problem. 
%
Then we provide an overview of \modelname. %~, which consists of two modules, i.e., dual dynamic graph modeling and hybrid metric training, along with the motivation behind each module.
%
Finally, we present the detailed components.
%

\subsection{Problem Formulation}

\ccc{intra/inter}
CDSR aims at exploring a set of common users' sequential preference with given historical behavior sequences during the same time period from multiple domains.
%
Without loss of generality, we take two domains (A and B) as example, and formulate the CDSR problem as follows. 
%
We represent two single-domain behavior sequences from a user as $S_A =\{A_1,A_2,...,A_i,...\}$ and $S_ B=\{B_1,B_2,...,B_j,...\}$, where $A_i \in \mathbb{A} (1 \leq i \leq n)$ is the index of one consumed item in domain A; $\mathbb{A}$ is the item index in domain A; and $B_i \in \mathbb{B}(1 \leq j \leq m)$ is the index of one consumed item in domain B; $\mathbb{B}$ is the item set in domain B. \ccc{rewrite}
%
Then the cross-domain behavior sequence $S$ is produced by merging $S_A$ and $S_B$ according to the chronological order, for which a specific example can be given as $S = \{A_1,B_1,B_2,...,A_i,B_j,...\}$.
%
Given $S$, CDSR tries to predict the next item by computing the recommendation probabilities for all candidates in two domains respectively : \ccc{}
%
\begin{equation}
\begin{aligned}
P(A_{i+1}|S_A,S_B,S) \sim f_A(S_A,S_B,S;\Omega^A), \\
P(B_{j+1}|S_B,S_A,S) \sim f_B(S_B,S_A,S;\Omega^B),
\nonumber
\end{aligned}
\end{equation}
%
where $P(A_{i+1}|S_A,S_B,S)$ denotes the probability of $A_{i+1}$ that will be consumed next in domain A, given $S_A$ and $S_B$. $f_A(S_A,S_B,S;\Omega^A)$ is the learned function to estimate $P(A_{i+1}|S_A,S_B,S)$.
%
Here $\Omega^A$ and $\Omega^B$ denote the parameters in the modeling structure of domain A and domain B, respectively.
%
Similar definitions can be applied to $P(B_{j+1}|S_B,S_A,S)$ and $f_B(S_B,S_A,S;\Omega^B)$.
\ccc{is is necessary?}

\subsection{An overview of \modelname }

%
% The aim of \modelname~is to learn a graphical recommendation model that can explore in-domain specific user interests as well as cross-domain invariant user interests in dual graphs, i.e., the local graph and the global graph, and meanwhile apply a gating mechanism to transfer knowledge from global feature space to local feature space. \ccc{too much information here}
The aim of \modelname~is providing better sequential recommendation performance for a single domain by leveraging useful cross-domain knowledge.
%
The overall structure of our proposed \modelname~ is illustrated in Figure \ref{fig:framework}. 
% To do this, we should firstly explore inter-domain preference features as well as intra-domain features in parallel, then transfer the information recurrently at each timestamp.
%
% Though cross-domain information has been utilized, the data sparsity problem still exist.
%
% Therefore, we enhance sequential representations in each domain with hybrid metric learning in prediction so that further promote recommendation performance.
% The construction of three graphs is achieved in a parallel and dynamic way, which means the information from both domains is shared recurrently at each timestamp. \ccc{relation with context}
%
\modelname~ consists of two main modules: (1) \textit{dual dynamic graph modeling} and (2) \textit{hybrid metric training}.
%
In the dual dynamic graph modeling module, we want to explore intra-domain preference features as well as inter-domain features in parallel, then transfer the information recurrently at each timestamp.
%
Thus, this module has two parts, i.e., \textit{dual graph construction} and \textit{fuse attentive gate}.
%
In the dual graph construction part, we build two-level directed graphs : a) \textit{local dynamic graph} for extracting \textit{intra-domain} transitions; b)\textit{global dynamic graph} for extracting \textit{inter-domain} transitions.
%
After it, we propose a fuse attentive gate which adopts attention mechanism to integrate item embeddings from global graph into local graph.
%
To this end, cross-domain information is effectively leveraged to enrich the single domain sequence representations.
%
Later, the sequential representations that combine intra-domain and inter-domain features are sent into the hybrid metric training module.

%
Though cross-domain information has been utilized, the data sparsity problem still exists.
%
\ccc{Thus, we propose xxx in the hybrid metric training module.}
Thus, except for the basic prediction, hybrid metric training module is innovatively designed for optimizing representation learning to reduce data sparsity impact.
%
The representation enhancement is twofold : a) adopt collaborative metric learning to realize alignment between similar instance representations; b) employ contrastive metric learning to preserve uniformity within different representation distributions.  
% is composed of two tasks, i.e., \textit{collaborative learning} for distinguishing positive and negative user-item joint metric and \textit{contrastive learning} for enhancing diverse user representations.
%
Finally, the model outputs the probability of each item to be the next click and generates a list of recommended items for both domains. 


\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{pic/model.png}
% \vspace{-0.3cm}
\caption{An overview of \modelname~. Local dynamic graph for domain $A$ is shown in orange, domain $B$ is shown in blue, and global dynamic graph is shown in gray. Section 3.2 contains a walkthrough of the model. 
}
\label{fig:framework}
% \vspace{-0.4cm} 
\end{figure*}

% \begin{algorithm}[htbp]
% \begin{algorithmic}[1]
% {
%     \STATE {
%     \textbf{Input:} $K$: Number of clusters; $\mathcal{N}(\boldsymbol{\breve{\mu}}^\mathcal{S}_c,(\boldsymbol{\breve{\sigma}}^\mathcal{S}_c)^2)$: The source user latent distribution for the $c$-th cluster group; $\mathcal{N}(\boldsymbol{\breve{\mu}}^\mathcal{T}_c,(\boldsymbol{\breve{\sigma}}^\mathcal{T}_c)^2)$: The target user latent distribution for the $c$-th cluster group; $\epsilon$: Hyper parameter to balance the matching loss and the entropy maximization constraint.
%     }
%     \STATE {
%     Initialize the coupling matrix $\boldsymbol{\psi}$.
%     }
%     \FOR{$i=1$ to $T$}
%     \STATE {Calculate the distance between different Normal distribution in source and target domains as matrix ${\mathcal{M}} \in \mathbb{R}^{K \times K \times K \times K}$ through Equation \eqref{equ:get_m}.}
%     \STATE {Calculate matrix $\mathcal{G} = {\mathcal{M}} \otimes \boldsymbol{\psi}$ and $\boldsymbol{H} = \exp \left( -\frac{\mathcal{{G}}}{\epsilon}\right)$. }
%     \STATE {Randomly initialize vectors $\boldsymbol{u}\in \mathbb{R}^K$ and $\boldsymbol{v}\in \mathbb{R}^K$.}
%         \FOR{$j=1$ to $t$}
%             \STATE {Update $\boldsymbol{u}  \leftarrow \boldsymbol{\pi}^{\mathcal{S}} \oslash (\boldsymbol{H}\boldsymbol{v})$. }
%             \STATE {Update $\boldsymbol{v} \leftarrow \boldsymbol{\pi}^{\mathcal{T}} \oslash (\boldsymbol{H}^{\top}\boldsymbol{u})$. }
%         \ENDFOR
%         \STATE{$\boldsymbol{\psi} = {\rm diag}(\boldsymbol{u}) \boldsymbol{H} {\rm diag}(\boldsymbol{v})$. }
%     \ENDFOR
%     \STATE{\textbf{Return}: $\boldsymbol{\psi}^* = \boldsymbol{\psi}$. }
% }
% \end{algorithmic}
% \caption{Dual Dynamic Graphs Modeling}
% \end{algorithm}

% \begin{algorithm}[t]
% \caption{Dual Dynamic Graph Modeling }\label{alg:dual-dynamic-graph-algo}
% \KwIn{user's cross-domain behavior sequence $S$;single-domain sequences: $S_A$,$S_B$.}
% \KwOut{Item embeddings in local domain graphs : $H_{Al}$, $H_{Bl}$; Sequential embeddings : $SE_{Al}$, $SE_{Bl}$ }
% {
% Initialize node embeddings in local graphs as $H^0_{Al}$ and $H^0_{Bl}$.\\
% Global node embeddings $H^0_g = H^0_{Al} \oplus H^0_{Bl}$ \\
% \textbf{for} $t=0$ to $T$ \textbf{do}\\
%     \quad Get the current item $v_{s,t}$, $v_{s,t}$'s domain as $X$; previous item in $S$ as $v_{s,t-1}$, in $S_X$ as $v_{s,t-1} $; previous item set as $V_{pre}$.\\
%     \quad \textbf{From global graph $\mathcal{G}^{t-1}_S$:} \\
%     \quad Select $V_{pre}$'s neighbor set as $N_{s-pre}$.\\
%     \quad $Emb(V_{pre})=h^{t-1}_{xg,pre}$, $Emb(N_{s-pre})=h^{t-1}_{xg,neig}$.\\
%     \quad Get global sequential embedding $SE^{t-1}_{xg}$ with Eq. (6-7).\\
%     \quad \textbf{From local graph $\mathcal{G}^{t-1}_X$:} \\
%     \quad $Emb(V_{pre})=h^{t-1}_{xl,pre}$.\\
%     \quad Get local sequential embedding $SE^{t-1}_{xl}$ with Eq. (6-7).\\
%     \quad \textbf{Do Fuse Attentive Gating:}\\
%     \quad\quad $\overline{h^{t-1}_{xl,pre}}$ = \textbf{GATE} ($h^{t-1}_{xg,pre}$ $h^{t-1}_{xl,pre}$, $h^{t-1}_{xg,neig}$, $SE^{t-1}_{xg}$, $SE^{t-1}_{xl}$) \\
%     \quad \textbf{On local graph $\mathcal{G}^t_X$ do:} \\
%     \quad\quad Update $V_{pre}$'s embeddings to new state $\overline{h^{t-1}_{xl,pre}}$\\
%     \quad\quad Add a directed edge from $v_{x,t-1}$ to $v_{x,t}$. \\
%     \quad\quad Update nodes on graph $\mathcal{G}^t_X$ with Eq. (1-5).\\
%     \quad \textbf{On global graph $\mathcal{G}^t_S$ do:} \\
%     \quad\quad Add a directed edge from $v_{s,t-1}$ to $v_{s,t}$. \\
%     \quad\quad Update nodes on graph $\mathcal{G}^t_S$ with Eq. (1-5).\\

% \textbf{end for}\\
% Get sequential embeddings $SE_{Al}$, $SE_{Bl}$ with Eq. (7-9).\\
% \textbf{return} $H_{Al}$, $H_{Bl}$; $SE_{Al}$, $SE_{Bl}$\\
% }
% \end{algorithm} 


\subsection{Dual Dynamic Graph Modeling}

The prime task for solving the CDSR problem is exploiting the expressive sequencial representations to depict user interests from the cross-domain behavior sequences.
%
Here, we propose a dual dynamic graph modeling module that extracts the latent item embeddings in both local and global graphical space, as is shown in in Appendix \ref{alg:dual-dynamic-graph-algo}. \ccc{where?}
%



\subsubsection{Dual graph construction}

To begin with, we first introduce how to construct the dual graphs.
%
There are two components in the architecture: (1) local dynamic graph for encoding intra-domain transitions; (2) global dynamic graph for encoding inter-domain transitions.

\ccc{link with fig. 2}
\nosection{Local dynamic graph}
In this part, we apply a dynamic gated GNN to capture the intra-domain sequential transitions that represent user preference patterns in each single domain \cite{wu2019session, zhang2022dynamic}.
% Inspired by \cite{wu2019session} and \cite{zhang2022dynamic}, to capture the intra-domain sequential transitions, we apply a dynamic gated GNN to compute embeddings for items.
%
Here we take domain $A$ as example.
%
Let $V_A = \{v_{a,1},v_{a,2},...,v_{a,N_a}\}$ denotes the set consisting of all unique items in domain $A$. \ccc{typo, why}
%
Then an sequence can be represented by a list $S_A = [v_{s,1},v_{s,2},...,v_{s,n_s}]$ ordered by timestamps, where $v_{s,i} \in V_A$ represents a consumed item of the user within the sequence $s_A$. \ccc{}
%
The local dynamic network $\mathcal{A}$ can be defined as a set $\{\mathcal{G}^1_A,\mathcal{G}^2_A,...,\mathcal{G}^T_A\}$ where $\mathcal{G}^t_A=\{\mathcal{V}^t_A,\mathcal{E}^t_A\}$ is the graph at snapshot $t$. \ccc{T?}
%
$\mathcal{V}^t_A$ is the set of nodes in $\mathcal{G}^t_A$ that indicates item representations, and $\mathcal{E}^t_A$ is the set of edges in $\mathcal{G}^t_A$ that shows the transitions between items.
%
When the user of the sequence $S_A$ acts on the item $v_{s,i}$ at time $t$, an edge $e$ is established from $v_{s,i-1}$ to $v_{s,i}$.
%
We embed every item $v \in V_A$ into an unified embedding space and the node vector $ h \in \mathbb{R}^N$ indicates the latent vector of item $v$ learned via graph neural networks, where $N$ is the dimensionality.
%

Then we demonstrate the learning process of node vectors in every $\mathcal{G}^t_A$ at snapshot $t$.
%
We extract node embeddings with GRU mechanism which unrolls the recurrence for a fixed number of steps $K$. \ccc{K?}
% Compared with normal GNNs, the biggest modification of Gated Graph Neural Networks (GG-NNs) \cite{li2015gated} is that we use Gated Recurrent Units (GRU) and unroll the recurrence for a fixed number of steps $K$.
% and use backpropagations through time in compute gradients.
%
So for the node $v_{s,i}$ of graph $\mathcal{G}^t_A$, the recurrence of the propagation functions are given as follows:

\begin{align}
\label{equ:prop}
a^k_{s,i} &= A_{s,i:}[h^{k-1}_1,...,h^{k-1}_n]^\top\mathbf{W}_h+\mathbf{b},\\
\label{equ:zgate}
z^k_{s,i} &= \sigma(\mathbf{W}_z a^k_{s,i}+\mathbf{U}_z h^{k-1}_i),\\
\label{equ:rgate}
r^k_{s,i} &= \sigma(\mathbf{W}_r a^k_{s,i}+\mathbf{U}_r h^{k-1}_i),\\
\label{equ:h4}
\widetilde{h^k_i} &= \tanh(\mathbf{W}_o a^k_{s,i}+\mathbf{U}_o(r^k_{s,i} \odot h^{k-1}_i)),\\
\label{equ:h5}
h^k_i &= (1-z^k_{s,i})\odot h^{k-1}_i+z^k_{s,i}\odot\widetilde{h^k_i},
\end{align}
where $[h^{k-1}_1,...,h^{k-1}_n]$ is the node embedding list in the current sequence and $k$ denotes the propagation step.
%
The matrix $A_s \in \mathbb{R}^{n \times 2n}$ is the concatenation of two adjacency matrices $A^{in}_s$ and $A^{out}_s$, which represents weighted
connections of outgoing and incoming edges in the $\mathcal{G}^t_A$ at snapshot $t$ respectively.
%
And $A_{s,i:}$ are the two columns of blocks in $A_{s}$ corresponding to node $v_{s,i}$. which describes how nodes in the graph communicate with each other.
%
The sparsity structure and parameter tying in $A_s$ is illustrated in Appendix \ref{fig:example-a} as an example. 
% \begin{figure}[t]
%  \begin{center}
%  \includegraphics[width=\columnwidth]{pic/example-aa.png}
%  \vspace{-0.2 in}
%  \caption{(a) and (b) are sequential graphs and corresponding connection matrices at timestamp $t$ and $t+1$.}
%  \vspace{-0.15 in}
%  \label{fig:example-a}
%  \end{center}
% \end{figure}
%
Eq. \eqref{equ:prop} shows the step that passes information between different nodes of the graph via edges in both directions. 
%
After that, a GRU-like update, including update gate $\mathbf{z}_{s,i}$ in Eq. \eqref{equ:zgate} and reset gate $\mathbf{r}_{s,i}$ in Eq. \eqref{equ:rgate}, is adopted to determine what information to be preserved and discarded respectively. 
%
$\sigma(\cdot)$ is the sigmoid function and $\odot$ is the element-wise multiplication operator. 
%
Then the candidate state is generated by the previous state, the current state under the control of the reset gate in Eq. \eqref{equ:h4}.
%
We combine the previous hidden state with the candidate state using updating mechanism and get the final state in Eq. \eqref{equ:h5}.
%

After $K$ steps of updating, we can obtain the embeddings of all nodes at each snapshot in local dynamic graph set $\{\mathcal{G}^1_A,\mathcal{G}^2_A,...,\mathcal{G}^T_A\}$ as $H_{Al}=\{H^1_{Al},H^2_{Al},...,H^T_{Al}\}$, where $H^t_{Al} = \{h^t_{al,1},h^t_{al,2},...,h^t_{al,i}\}$.
%
Besides, we consider the sequence embedding $SE^t_{Al}$ for $\mathcal{G}^t_A$ by aggregating all node vectors.
%
Since information in these embedding may have difference levels of priority, we further adopt the soft-attention mechanism to better represent the complete sequence:
%
\begin{equation}
\begin{aligned}
\alpha^t_{al,k} &= p^\top_{al,t}\sigma(\mathbf{W}^t_{a1}h^t_{al,i}+\mathbf{W}^t_{a2}h^t_{al,k}+\mathbf{c}^t),\\
SE^t_{Ac} &= \sum_{k=1}^i\alpha^t_{a,k}h^t_{al,k},
\end{aligned}
\end{equation}
%
where parameters $p^\top_{a,t} \in \mathbb{R}^d$ and $\mathbf{W}^t_{a1},\mathbf{W}^t_{a2} \in \mathbb{R}^{d \times d}$ control the weights of item embedding vectors.
%
Then, the final sequence embedding $SE^t_{Al}$ is computed by taking linear transformation over the concatenation of the last item embedding and the complete sequence embedding:
%
\begin{equation}
\begin{aligned}
SE^t_{Al} = \mathbf{W}^t_{a3}[SE^t_{Ac};h^t_{al,i}].
\end{aligned}
\end{equation}
%
Correspondingly, the node embeddings in local dynamic graph of domain $B$ are denoted as $H_{Bl}=\{H^1_{Bl},H^2_{Bl},...,H^T_{Bl}\}$, and the corresponding sequence embeddings at each timestamp $t$ is achieved as $SE^t_{Bl}$.
%

\nosection{Global dynamic graph}
Except inter-domain sequential transitions , it is also a necessity to model inter-domain transitions so as to leverage the knowledge from other domains.
%
To this end, we apply the global dynamic graph to capture diverse trends of user preference in a shared latent feature space.
%
The dynamical construction of the global graph is similar to the local graph described above, the only difference is that the modeling target becomes the merged sequence, such as $S = \{A_1,B_1,B_2,...,A_i,B_j,...\}$.
%
Specifically, the initial embeddings of items in the global graph are adopted from two local embedding spaces accordingly at the beginning.
%
As the user of the merged sequence acts on the items from two domains, we add the directed edges continuously and consequently get a set of graphs as $\{\mathcal{G}^1_S,\mathcal{G}^2_S,...,\mathcal{G}^T_S\}$ with the state of all nodes as $H_{g}=\{H^1_{g},H^2_{g},...,H^T_{g}\}$ after propagating.
%
Then item embeddings from domain $A$ and domain $B$ in this shared space could be extract from $H_{g}$, defined as $H_{Ag}=\{H^1_{Ag},H^2_{Ag},...,H^T_{Ag}\}$ and $H_{Bg}=\{H^1_{Bg},H^2_{Bg},...,H^T_{Bg}\}$ respectively.
%
And the sequence embeddings on the global graph at each timestamp $t$ for two domain can be obtained as $SE^t_{Ag}$ and $SE^t_{Bg}$.
 
\ccc{link with fig. 3}
\subsubsection{Fuse Attentive Gate}

% On the other hand, the time intervals of successive items exert a major influence on how much an item's representation reflects the user interest.
% %
% Thus, combining the item features in dual space in a time-aware way is as well crucial to precisely capture users' short-term and long-term interests.
% %
In this part, we introduce how to build the transferring bridge between the local graphs and the global graph.
%
% once an user-item interaction happens, only the structure of the global graph and the local graph where item belongs to varies.
%
The challenges in transferring lay in two folds : (1) users' general evolving interest patterns in dual feature spaces should be incorporated both in item-level and sequence-level. 
%
(2) Due to the structured encoding technique used in graph modeling, the neighboring field influence should also be considered in transferring to avoid loss of context information. \sjj{check}

% On the one hand, the transferring process should not only be item-level but also sequence-level so that users' general evolving interest patterns in dual feature spaces can be better incorporated.
%
% On the other hand, due to the structured encoding technique used in dual graph modeling, the neighboring field influence should be considered in transferring to avoid loss of context information.\sjj{too long}
% since item nodes in two graphs are proceeded simultaneously, only selecting the nodes that appear in the current local graph from global graph for transferring will cause loss of context information.
%

In tackle above issues, we innovatively propose a fuse attentive gate (FAG) to transfer the cross-domain information.
%
The structure of the gate is illustrated in Figure \ref{fig:gate}, and here we take the merged sequence $\{A_1,B_1,B_2,A_2,B_3,...\}$ for example.
%
At the timestamp $t$, $B_3$ is added into the graphs, the node embedding set that needs transferring from global graph to local graph in domain B is $\{B_1,B_2\}$.
%
Firstly, we take the sequence embedding $SE^{t-1}_{bg}$ from global graph and $SE^{t-1}_{bl}$ from local graph  at timestamp $t-1$ to achieve the sequence-aware fusion:
%
\begin{equation}
\begin{aligned}
    \mathbf{W}^t_{att} = \mathbf{W}^t_{gen}[SE^{t-1}_{bg},SE^{t-1}_{bl}]+\mathbf{b}^t_{gen}.
\nonumber
\end{aligned}
\end{equation}
%
Intuitively, we should consider two aspects of feature aggregation, i.e., \textit{self-attentive} and \textit{neighbour-attentive} aggregation.
%
The self-attentive aggregation is to combine the global node embedding $h^{t-1}_{bg,x}$ and the local node embedding $h^{t-1}_{bl,x}$ for retaining own features:
%
\begin{equation}
\begin{aligned}
    \mathbf{\alpha}_{self-l} &= (\mathbf{W}^t_{self})^\top \tanh(\mathbf{W}^t_{att}[h^{t-1}_{bl,x},h^{t-1}_{bl,x}]), \\
    \mathbf{\alpha}_{self-g} &= (\mathbf{W}^t_{self})^\top \tanh(\mathbf{W}^t_{att}[h^{t-1}_{bl,x},h^{t-1}_{bg,x}]), \\
    \widetilde{h^t_{bl,x}} &= \mathbf{\alpha}_{self-l}\cdot h^{t-1}_{bl,x}+\mathbf{\alpha}_{self-g}\cdot h^{t-1}_{bg,x}.
\nonumber
\end{aligned}
\end{equation}
The neighbour-attentive aggregation is to transfer the influence of message passing from global neighbours $N(bg,x)$ so that further enhance the representation of the local node $x$:
%
\begin{equation}
\begin{aligned}
    \mathbf{\alpha}^i_{neig} &= \frac{exp((h^{t-1}_{bl,x})^\top\mathbf{W}^t_{att}h^{t-1}_{bg,i})}{\sum_{i \in N(bg,x)}exp((h^{t-1}_{bl,x})^\top\mathbf{W}^t_{att}h^{t-1}_{bg,i})}, \\
    \widehat{h^t_{bl,x}} &= \sum_{i \in N(bg,x)} \mathbf{\alpha}^i_{neig}\cdot h^{t-1}_{bg,i}.
\nonumber
\end{aligned}
\end{equation}
%
With self-aware feature $\widetilde{h^t_{bl,x}}$ and neighbour-aware feature $\widehat{h^t_{bl,x}}$, we then employ a GRU-based gating mechanism as the recurrent unit:
\begin{equation}
\begin{aligned}
    z_{gate} &= \sigma(\mathbf{W}_{gz}[\widehat{h^t_{bl,x}},\widetilde{h^t_{bl,x}}]),\\
    r_{gate} &= \sigma(\mathbf{W}_{gr}[\widehat{h^t_{bl,x}},\widetilde{h^t_{bl,x}}]),\\
    h_{gate} &= \tanh(\mathbf{W}_{gh}[\widehat{h^t_{bl,x}},r_{gate}\odot \widetilde{h^t_{bl,x}}],\\
    \overline{h^t_{bl,x}} &= (1-z_{gate})\odot\widetilde{h^t_{bl,x}}+z_{gate}\odot h_{gate},
\nonumber
\end{aligned}
\end{equation}
%
where $\mathbf{W}_{gz}$,$\mathbf{W}_{gr}$ and $\mathbf{W}_{gh}$ are weight matrices. $\overline{h^t_{bl,x}}$ is the output of the fuse attentive gate which represents the updated state at timestamp $t$ of the nodes on the local graph after transferring.

\begin{figure}[t]
 \begin{center}
 \includegraphics[width=\columnwidth]{pic/gate.png}
%  \vspace{-0.2 in}
 \caption{The structure of the Fuse Attentive Gate. Here $\oplus$ means concatenation, $\times$ means element-wise multiplication, and $+$ means addition.\sjj{add description into pic}}
%  \vspace{-0.15 in}
 \label{fig:gate}
 \end{center}
\end{figure}



\subsection{Hybrid Metric Training}

With final representations of sequences from domain $A$ and $B$, hybrid metric training module evaluates the recommendation probabilities of the candidate items. 
% \ccc{simply summarize it first}
%
This module mainly has two purposes, including (1) exploring user preference for different items in two domains, which is the prime purpose of the model, (2) alleviate the remaining data sparsity problem. 
%
% (2) capturing diverse user-item and item-item relationships; (3) extracting meaningful user patterns and enhancing user representations.
% To achieve these purposes, except for the basic prediction function that existing researches always adopt, we additionally employ two aspects of controls, i.e., collaborative loss control and contrastive loss control, to optimize the performance of recommendation.
As for the first purpose, we apply basic prediction function that existing researches always adopt.
%
To achieve the second purpose, we optimize representation learning process with two enhancements, i.e., collaborative metric for retaining representation alignment and contrastive metric for preserving uniformity, thus further improve recommendation performance.
%


\nosection{Basic Prediction}
As most existing researches, we firstly calculate the matching between sequence-level embeddings $SE_{Al}$, $SE_{Bl}$ and corresponding domain item-embedding matrices $H_{Al}$, $H_{Bl}$ to compute the recommendation probabilities:\sjj{notations}
%
\begin{equation}
\begin{aligned}
    P(A_{i+1}|S_A,S_B) &= softmax(H_{Al}\cdot SE_{Al}^\top + b_A),\\
    P(B_{j+1}|S_B,S_A) &= softmax(H_{Bl}\cdot SE_{Bl}^\top + b_B),
\nonumber
\end{aligned}
\end{equation}
%
where $b_A$ and $b_B$ are bias items.
%
Then negative log-likelihood loss function is employed as follows:
%
\begin{equation}
\begin{aligned}
    \mathcal{L}_A &= -\frac{1}{|\mathbb{S}|}\sum_{S \in\mathbb{S}}\sum_{A_i \in S}\log P(A_{i+1}|S_A,S_B),\\
    \mathcal{L}_B &= -\frac{1}{|\mathbb{S}|}\sum_{S \in\mathbb{S}}\sum_{B_j \in S}\log P(B_{j+1}|S_B,S_A),
\nonumber
\end{aligned}
\end{equation}
%
$\mathbb{S}$ denotes the training sequences in both domains.
%

%
% \sjj{
% However, the above objective function models users' preference towards items solely based on user-item similarity, but overlooks the relations between user-user and item-item representation pairs.
% %
% Besides, since the dual dynamic graph modeling mainly focusing on depicting accurate feature embeddings on item-level, how to enhance representations on user behavior sequence level to alleviate data sparsity problem remains a key issue.
% }
%
% To address these problems, we additionally employ two aspects of constraints, i.e., collaborative loss and contrastive loss, to further optimize the performance of recommendation.



\nosection{Collaborative Metric} 
The collaborative metric aims to achieve representation alignment, which means that similar instance are expected to have similar representations.
%
Here we model the observed item sequence as a set of positive user-item pairs $\mathcal{T}_\mathcal{S}$ and learn a user-item join metric to encode these relationships \cite{hsieh2017collaborative}. 
%
And the set of sequences in current batch is denoted as $\mathcal{S}$.
%
Specifically, the learned metric pulls the pairs in $\mathcal{T}_\mathcal{S}$ closer and pushes the other pairs relatively further apart.
%
This process, due to the triangle inequality, will also cluster a) the users who co-interact with the similar item sequence together, and b) the items that are co-liked by the same users together.
%

Concretely, we learn the model parameters by optimizing the large margin nearest neighbor objective (LMNN) \cite{park2018collaborative} as follows
%
\begin{equation}
\begin{aligned}
    \mathbf{W}^{rank}_{ij} &= log(rank_D(i,j)+1),\\
    \mathcal{L}_{col}(\mathcal{S}) &= \sum_{(i,j)\in\mathcal{T}_\mathcal{S}}\sum_{(i,j)\notin\mathcal{T}_\mathcal{S}}\mathbf{W}^{rank}_{ij}[m+D(i,j)^2-D(i,k)^2]_+,
\nonumber
\end{aligned}
\end{equation}
% 
where $j$ is the item in historical sequences of user $i$, $k$ is an item never appears in these sequences.
%
Specifically, $\mathbf{W}^{rank}_{ij}$ is a rank-based loss weight adopted from Weighted Approximate-Rank Pairwise (WARP) loss \cite{weston2010large}.
%
Given metric $D$, let $J$ denotes the total number of items and $rank_D(i,j)$ denotes the rank of item $j$ in user $i$’s recommendations.
%
$D$ is defined as euclidean distance between user i and item j as $D(i,j) = \parallel SE_{*l,i}-h_{*l,j}\parallel$, where $SE_{*l,i}$ is final sequence embeddings representing user preference and $h_{*l,j}$ is item embeddings in the final local graph.
%
$*$ indicates the domain name as $A$ or $B$.
%
$m>0$ means the safety margin between positive pairs and negative pairs.
%
% Given metric $D$, let $J$ denotes the total number of items and $rank_D(i,j)$ denotes the rank of item $j$ in user $i$’s recommendations, we penalize a positive item $j$ based on its rank by setting:
%
% \begin{equation}
% \begin{aligned}
%     \mathbf{W}^{rank}_{ij} = log(rank_D(i,j)+1).
% \nonumber
% \end{aligned}
% \end{equation}
%
% Actually, to utilize the massive parallelism enabled by modern GPUs, we usually take the negative-sampling scheme and $rank_D(i,j)$ is then approximated as $\lfloor\frac{J \times M}{U} \rfloor$, where $M$ denote the number of imposts in $U$ negative samples. \sjj{not concise}
%


\nosection{Contrastive Metric}
The contrastive metric aims to realize representation uniformity, which means the distribution of representations is preferred to preserve as much information as possible.
% Inspired by the SimCLR framework \cite{chen2020simple} for learning visual representation, we seek to explore applying contrastive learning to CDSR task to enhance user representations.
%
To do this, the contrastive loss learns to minimize the difference between differently augmented views of the same user historical sequence and maximize the difference between the augmented sequences derived from different users.
%

Here we apply a random \textit{Item Mask} as the augmentation operator.
%
We take domain A for example.
%
For each user historical sequence $S_{A,u}$, we randomly mask a proportion of items and and denote the masked sequence as $S^{mask}_{A,u}$.
% $\gamma$ of items $\mathscr{M}_{S_{A,u}}=(m_1,m_2,...,m_{L_a})$ with the length $L_a=\lfloor\gamma*|S_{A,u}|\rfloor$ and $m_i$ is the index of items in $S_{A,u}$ which will be masked.
% %
% Then this augmentation method can be formulated as:
% %
% \begin{equation}
% \begin{aligned}
%     S^{mask}_{A,u} &= [\widehat{A_1},\widehat{A_2},...\widehat{A}_{|S_{A,u}|}],\\
%     \widehat{A_t} &= \left\{
% \begin{array}{rcl}
% A_t       &      & t\in \mathscr{M}_{S_{A,u}};\\
% \left[mask]\right.       &      & t\notin \mathscr{M}_{S_{A,u}}.
% \end{array} \right.
% \nonumber
% \end{aligned}
% \end{equation}
%
For a mini-batch of N users $\{u_1,u_2,...u_N\}$, we apply augmentation to each user's sequence and obtain 2$N$ sequences $\left[S_{A,u_1},S^{mask}_{A,u_1},S_{A,u_2},S^{mask}_{A,u_2},...,S_{A,u_n},S^{mask}_{A,u_n}]\right.$
%
For each user $u$, we treat $(S_{A,u},S^{mask}_{A,u})$ as the positive pair and treat other $2(N-1)$ examples with the same mini-batch as negative samples $S^-$.
%
We utilize dot product to measure the similarity between each representation, $sim(u,v)=u^\top v$.
%
Then the contrastive loss function can be defined to the widely used softmax cross entropy loss as:
%
\begin{equation}
\begin{aligned}
    \mathcal{L}_{con}(\mathcal{S}) = \sum_{\mathcal{P} \in \mathbb{P}_S} - \frac{1}{|\mathcal{P}|} \sum_{(x,y)\sim\mathcal{P}}log \frac{exp(sim(SE_x,SE_y)/\tau)}{\sum_{x^{'}\in\{y\}\cup \mathcal{X}^-_\mathcal{P}}exp(sim(SE_x,SE_{x^{'}})/\tau)}.
\nonumber
\end{aligned}
\end{equation}
%
$\mathbb{P}_S$ is the set of positive pairs, and $\mathcal{X}^-_\mathcal{P}$ is the sampled negative item set for $\mathcal{P}$.
%
$\tau$ is a temperature parameter.

\nosection{Putting Together}
Finally, we join recommendation objectives in two domains with collaborative and contrastive enhancement together via a multi-task training scheme:
%
\begin{equation}
\begin{aligned}
\mathcal{L} = \mathcal{L}_A + \mathcal{L}_B + \lambda _{col}\mathcal{L}_{col} + \lambda_{con}\mathcal{L}_{con},
\nonumber
\end{aligned}
\end{equation}
where $\lambda_{col}$ and $\lambda_{con}$ are hyper-parameters to balance different type of losses.
% \ccc{explain hyper-parameters.}






